Mock Deep Testing: Toward Separate Development of Data and Models for Deep Learning

While deep learning (DL) has permeated, and become an integral component of many critical software systems, today software engineering research hasn't explored how to separately test data and models that are integral for DL approaches to work effectively. The main challenge in independently testing these components arises from the tight dependency between data and models. This research explores this gap, introducing our methodology of mock deep testing for unit testing of DL applications. To enable unit testing, we introduce a design paradigm that decomposes the workflow into distinct, manageable components, minimizes sequential dependencies, and modularizes key stages of the DL. For unit testing these components, we propose modeling their dependencies using mocks. This modular approach facilitates independent development and testing of the components, ensuring comprehensive quality assurance throughout the development process. We have developed KUnit, a framework for enabling mock deep testing for the Keras library. We empirically evaluated KUnit to determine the effectiveness of mocks. Our assessment of 50 DL programs obtained from Stack Overflow and GitHub shows that mocks effectively identified 10 issues in the data preparation stage and 53 issues in the model design stage. We also conducted a user study with 36 participants using KUnit to perceive the effectiveness of our approach. Participants using KUnit successfully resolved 25 issues in the data preparation stage and 38 issues in the model design stage. Our findings highlight that mock objects provide a lightweight emulation of the dependencies for unit testing, facilitating early bug detection. Lastly, to evaluate the usability of KUnit, we conducted a post-study survey. The results reveal that KUnit is helpful to DL application developers, enabling them to independently test each component effectively in different stages.

==> results.tex <==

\begin{table*}[]
\caption{Comparision of issues detected by KUnit before integration and DeepDiagnosis~\cite{wardat22DeepDiagnosis} after integration}
\huge
% \scalebox{0.67}{
\begin{adjustbox}{width=\textwidth,center}

\begin{tabular}{|c|c|l|l|l|l|}

\hline
\rowcolor[HTML]{C0C0C0} 
\cellcolor[HTML]{C0C0C0}                                & \cellcolor[HTML]{C0C0C0}                                                                                    & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}}                                                                                                         & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Issues Detected in Data Preparation Stage}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Issues Detected in Model Building Stage}}                                                                                                                                                                                                                                                                                                                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Issues Detected by DeepDiagnosis}}                                                                                                                                                           \\ \cline{4-6} 
\rowcolor[HTML]{C0C0C0} 
\multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{SO\#}} & \multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Type \\  of Task\end{tabular}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{Issues Identified by SOF User}}}                                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Before Integration using Mock Model}}       & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Before Integration using Model Data}}                                                                                                                                                                                                                                                                                                                                           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{After Integration}}                                                                                                                                                                          \\ \hline
31627380                                                & BC                                                                                                          & \begin{tabular}[c]{@{}l@{}}Wrong Output Layer Activation\\  Wrong Loss Function\end{tabular}                                                          & AssertionError('Data is not normalized or scaled',)                                             & \begin{tabular}[c]{@{}l@{}}AssertionError('Incorrect loss --\textgreater \\ Use binary crossentropy',)\\ AssertionError('Incorrect output layer activation --\textgreater \\ Use sigmoid  activation',)\end{tabular}                                                                                                                                                                                                                & \begin{tabular}[c]{@{}l@{}}Batch 0 layer 3: Numerical Error in delta Weights, \\  terminating training--- 0.9823560000000002 seconds ---		\\ Please change the loss function OR \\ Please change the activaton function at layer: 4\end{tabular} \\ \hline
\rowcolor[HTML]{C0C0C0} 
39525358                                                & BC                                                                                                          & Missing Scaling                                                                                                                                       & AssertionError('Data is not normalized or scaled',)                                             & No bug                                                                                                                                                                                                                                                                                                                                                                                                                              & \begin{tabular}[c]{@{}l@{}}Batch 19 layer 1: Dead Node Problem, \\  terminating training--- 13.167072000000001 seconds ---		 \\ Normalize the data\end{tabular}                                                                                  \\ \hline
48486598                                                & RG                                                                                                          & \begin{tabular}[c]{@{}l@{}}Missing Scaling\\  Missing Activations\\  Missing Evaluation Metrics\end{tabular}                                          & AssertionError('Data is not normalized or scaled',)                                             & \begin{tabular}[c]{@{}l@{}}AssertionError('Incorrect metrics --\textgreater \\ Use mean squared error or mean  absolute error',)\\ AssertionError('Missing non-linear activation function',)\end{tabular}                                                                                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}Batch 7: Invalid accuracy, \\  terminating training--- 2.36078 seconds ---	 	 \\ Please change the activation function at layer : 2\end{tabular}                                                                      \\ \hline
\rowcolor[HTML]{C0C0C0} 
60801900                                                & RG                                                                                                          & Wrong Output Layer Activation                                                                                                                         & No bug                                                                                          & \begin{tabular}[c]{@{}l@{}}AssertionError('Incorrect metrics --\textgreater \\ Use mean squared error or mean absolute error',)\\ AssertionError('Incorrect output layer activation --\textgreater \\ Use linear activation',)\end{tabular}                                                                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}Batch 0: Invalid accuracy, \\  terminating training--- 0.8810980000000002 seconds ---	 	 \\ Please change the activation function at layer : 5\end{tabular}                                                           \\ \hline
44066044                                                & BC                                                                                                          & \begin{tabular}[c]{@{}l@{}}Missing Scaling\\  Wrong Output Layer Activation\end{tabular}                                                              & AssertionError('Data is not normalized or scaled',)                                             & \begin{tabular}[c]{@{}l@{}}AssertionError('Incorrect output layer activation --\textgreater \\ Use sigmoid activation',)\end{tabular}                                                                                                                                                                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}Batch 0 layer 5: Numerical Problem Forward, \\  terminating training --- 0.6830479999999999 seconds ---		 \\  Normalize the data\end{tabular}                                                                         \\ \hline
\rowcolor[HTML]{C0C0C0} 
33969059                                                & RG                                                                                                          & Wrong Output Layer Activation                                                                                                                         & AssertionError('Data is not normalized or scaled',)                                             & \begin{tabular}[c]{@{}l@{}}AssertionError('Incorrect metrics --\textgreater \\ Use mean squared error or mean absolute error',)\\ AssertionError('Learning Rate too high: \\ Decrease the Learning Rate',)\\ AssertionError('Incorrect output layer activation --\textgreater \\ Use linear activation',)\end{tabular}                                                                                                              & \begin{tabular}[c]{@{}l@{}}Batch 0: Invalid accuracy, \\  terminating training--- 2.748129 seconds ---		 \\ Learning Rate\end{tabular}                                                                                                           \\ \hline
66840108                                                & RG                                                                                                          & \begin{tabular}[c]{@{}l@{}}Incorrect Input Shape\\  Wrong Output Layer Activation\\  Wrong Loss Function\\  Incorrect Evaluation Metrics\end{tabular} & AssertionError('Data is not normalized or scaled',)                                             & \begin{tabular}[c]{@{}l@{}}AssertionError('Mismatch in input shape',)\\ AssertionError({[}'Incorrect loss --\textgreater \\ Use mean squared error or mean absolute error'{]},)\\ AssertionError('Incorrect metrics --\textgreater \\ Use mean squared error or mean absolute error',)\\ AssertionError('Incorrect output layer activation --\textgreater \\ Use linear activation',)\end{tabular}                                  & \begin{tabular}[c]{@{}l@{}}Batch 0: Invalid accuracy, \\  terminating training--- 0.6627250000000002 seconds ---	 	 \\ Please change the activation function at layer : 2\end{tabular}                                                           \\ \hline
\rowcolor[HTML]{C0C0C0} 
46995209                                                & RG                                                                                                          & \begin{tabular}[c]{@{}l@{}}Missing Scaling\\  Wrong Activation Function\\  Wrong Output Layer Activation\end{tabular}                                 & AssertionError('Data is not normalized or scaled',)                                             & \begin{tabular}[c]{@{}l@{}}AssertionError('Incorrect metrics --\textgreater \\ Use mean squared error or mean absolute error',)\\ AssertionError('Incorrect output layer activation --\textgreater \\ Use linear activation',)\end{tabular}                                                                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}Batch 19: Accuracy Not Increasing, \\  terminating training--- 27.848416 seconds ---		 \\ Normalize the data\end{tabular}                                                                                             \\ \hline
68751439                                                & MC                                                                                                          & Incorrect Output Shape                                                                                                                                & AssertionError('Data is not normalized or scaled',)                                             & \begin{tabular}[c]{@{}l@{}}AssertionError('Mismatch in output shape --\textgreater \\ number of units should be same as number of classes',)\end{tabular}                                                                                                                                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}ValueError: Error when checking target: \\  expected dense\_4 to have shape (1,) \\  but got array with shape (11,)\end{tabular}                                                                                      \\ \hline
\rowcolor[HTML]{C0C0C0} 
41596619                                                & MC                                                                                                          & \begin{tabular}[c]{@{}l@{}}Wrong Output Layer Activation\\  Wrong Loss Function\end{tabular}                                                          & AssertionError('Data is not normalized or scaled',)                                             & \begin{tabular}[c]{@{}l@{}}AssertionError('Incorrect loss --\textgreater \\ Use categorical crossentropy',)\\ AssertionError('Incorrect output layer activation --\textgreater \\ Use softmax activation',)\\ AssertionError('Mismatch in output shape --\textgreater \\ number of units should be same as number of classes',)\\ AssertionError('Slow Convergence --\textgreater \\ Change Optimizer/Learning Rate',)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Batch 0: Invalid accuracy, \\  terminating training--- 0.424496 seconds ---	 	 \\ Please change the activation function at layer : 1\end{tabular}                                                                     \\ \hline
                                        
\end{tabular}
\label{SOFresults}
\end{adjustbox}
\end{table*}
